Hydrodynamic limit of the Symmetric Exclusion Process on a compact Riemannian manifold

We consider the symmetric exclusion process on suitable random grids that approximate a compact Riemannian manifold. We prove that a class of random walks on these random grids converge to Brownian motion on the manifold. We then consider the empirical density field of the symmetric exclusion process and prove that it converges to the solution of the heat equation on the manifold.

==> Summary.tex <==
\section*{Summary}
